A Bit of Nondeterminism Makes Pushdown Automata Expressive and Succinct

We study the expressiveness and succinctness of history-deterministic pushdown automata (HD-PDA) over finite words, that is, pushdown automata whose nondeterminism can be resolved based on the run constructed so far, but independently of the remainder of the input word. These are also known as good-for-games pushdown automata. We prove that HD-PDA recognise more languages than deterministic PDA (DPDA) but not all context-free languages (CFL). This class is orthogonal to unambiguous CFL. We further show that HD-PDA can be exponentially more succinct than DPDA, while PDA can be double-exponentially more succinct than HD-PDA. We also study HDness in visibly pushdown automata (VPA), which enjoy better closure properties than PDA, and for which we show that deciding HDness is ExpTime-complete. HD-VPA can be exponentially more succinct than deterministic VPA, while VPA can be exponentially more succinct than HD-VPA. Both of these lower bounds are tight. We then compare HD-PDA with PDA for which composition with games is well-behaved, i.e. good-for-games automata. We show that these two notions coincide, but only if we consider potentially infinitely branching games. Finally, we study the complexity of resolving nondeterminism in HD-PDA. Every HDPDA has a positional resolver, a function that resolves nondeterminism and that is only dependant on the current configuration. Pushdown transducers are sufficient to implement the resolvers of HD-VPA, but not those of HD-PDA. HD-PDA with finite-state resolvers are determinisable.

==> content/proofs.tex <==
\subsection{Proofs Omitted due to Space Restrictions}
\label{appendix_proofs}
\subsubsection{Proof of Lemma~\ref{lemma_inclusions}}

Recall that we need to prove \dcfl $\subseteq $ \gfgcfl $\subseteq$ \cfl.

\begin{proof}
We only consider the first inclusion, as the second one is trivial.
So, let $L \in $ \dcfl, say it is recognised by the DPDA~$\aut = (Q, \Sigma, \Gamma, q_\initmark, \Delta, F)$. 
We say that a mode~$m$ of $\aut$ is a reading mode if it does not enable an $\epsilon$-transition.
Hence, due to determinism, $m$ can only enable at most one $a$-transition for every $a \in \Sigma$.

Now, consider some nonempty word~$w(0) \cdots w(n) \in L(\aut)$ (we take care of the empty word later on), say with accepting run~$\rho$ (treated, for notational convenience, as a sequence of transitions).
This run can be decomposed as
\[\rho = \rho_0\, \tau_0\, \rho_1\, \tau_1\, \rho_2\, \cdots\, \rho_n\, \tau_n\, \rho_{n+1} \]
where $\tau_i$ processes $w(i)$ and each $\rho_i$ is a (possibly empty) sequence of $\epsilon$-transitions.
Each run prefix induced by some $\rho_0 \tau_0 \rho_1 \cdots \rho_{i}$ ends in a configuration with reading mode.

Intuitively, we have to eliminate the trailing $\epsilon$-transitions in $\rho_{n+1}$.
To do so, we postpone the processing of the letter~$w(i)$ to the end of $\rho_{i+1}$.
Instead, we guess that the next input is $w(i)$ by turning the original  $w(i)$-transition~$\tau_i$ into an $\epsilon$-transition $\tau_i'$ that stores $w(i)$ in the state space of the modified automaton. 
Then, $\rho_{i+1}$ is simulated, a dummy transition~$\tau_i^d$ processing the stored letter~$w(i)$ is executed. 

Hence, the resulting run of the modified automaton on $w$ has the form
\[\rho_0\, \tau_0'\, \rho_1\, \tau_0^d\, \tau_1'\, \rho_2\, \tau_1^d\, \cdots\, \rho_n\, \tau_{n-1}^d\, \tau_n'\, \rho_{n+1}\, \tau_n^d,\]
where each $\tau_i'$ is now an $\epsilon$-transition, each $\rho_i$ is a (possibly empty) sequence of $\epsilon$-transitions, and each $\tau_i^d$ is a dummy transition processing $w(i)$. 
Hence, the run ends with the transition processing the last letter $w(n)$ of the input. 


The resulting PDA is history-deterministic, as a resolver has access to the next letter to be processed, which is sufficient to resolve the nondeterminism introduced by the guessing of the next letter.

More formally, let PDA~$\aut' = (Q', \Sigma, \Gamma, q_\initmark', \Delta', F')$ where 
\begin{itemize}
    \item $Q' = Q \cup (Q \times \Sigma)$,
    \item $q_\initmark' = q_\initmark$,
    \item $F' = F \cup I$ where $I=\set{q_\initmark}$ if $\epsilon \in L(\aut)$ and $I = \emptyset$, otherwise, and
    \item $\Delta'$ is the union of the following sets of transitions:
    \begin{itemize}
        \item $\set{\tau \in \Delta \mid \ell(\tau) = \epsilon}$, which is used to simulate the leading sequence of $\epsilon$-transitions before the first letter is processed by $\aut$, i.e. the transitions in $\rho_0$ above.

        \item $\set{(q, X, \epsilon, (q',a),\gamma) \mid (q,X,a,q',\gamma) \in \Delta \text{ and } a\in \Sigma}$, which are used to guess and store the next letter to be processed. 

        \item $\set{((q,a), X, \epsilon, (q',a),\gamma) \mid (q,X,\epsilon,q',\gamma) \in \Delta }$, which are used to simulate $\epsilon$-transitions after a letter has been guessed, but not yet processed (i.e. transitions in some $\rho_i$ with $i>0$).
        
        \item $\set{ ((q,a), X, a, q, X) \mid (q,X) \text{ is a reading mode}}$, the dummy transitions used to actually process the guessed and stored letter.
        
    \end{itemize}
    
\end{itemize}

Now, formalising the intuition given above, one can show that $\aut'$ has a resolver witnessing that it recognises $L(\aut)$.
In particular, the empty word is in $L(\aut')$ if and only if it is in $L(\aut)$, as the run induced by the resolver on $\epsilon$ ends in the initial configuration, which is final if and only if $\epsilon \in L(\aut)$.
\end{proof}


\subsubsection{Proof of Theorem~\ref{theorem_closure}}

We need to prove the non-closure of \gfgcfl under union, intersection, complementation, set difference and homomorphism. Some of the proofs refer to results proven later in the appendix.

\begin{lemma} \label{closure_union}
\gfgcfl is not closed under union.
\end{lemma}

\begin{proof}
Consider the languages $L_1 = \{a^nb^n  \mid  n \geqslant 0\}$ and $L_2 = \{a^nb^{2n}  \mid  n \geqslant 0\}$ respectively. There exist a DPDA recognising $L_1$ and a DPDA recognising $L_2$.
Hence by Lemma~\ref{lemma_inclusions}, there also exist an \HD-PDA recognising $L_1$ and an \HD-PDA recognising $L_2$.
However, by Lemma \ref{lem:expressiveness1}, we have that $L_1 \cup L_2$ cannot be recognised by an \HD-PDA.
\end{proof}


\begin{lemma} \label{closure_intersection}
\gfgcfl is not closed under intersection.
\end{lemma}

\begin{proof}
Consider the languages $L_1 = \{a^nb^nc^m  \mid  m,n \geqslant 0\}$ and $L_2 = \{a^mb^nc^n  \mid  m,n \geqslant 0\}$.
There exist DPDA recognising $L_1$ and $L_2$.
Hence by Lemma \ref{lemma_inclusions} there exist \HD-PDA recognising $L_1$ and $L_2$.

Now let $L  = L_1 \cap L_2 = \{a^nb^nc^n  \mid  n \geqslant 0\}$.
As $L$ is not a \cfl  there does not exist any \HD-PDA recognising $L$.
\end{proof}

\begin{lemma} \label{closure_complementation}
\gfgcfl is not closed under complementation.
\end{lemma}

\begin{proof}
Recall the language
\begin{align*}
    B_2 &= \{a^i\$a^j\$b^k\$ \mid k \leqslant \max(i,j)\}.
\end{align*}
We proved with Lemma \ref{lem_expressiveness} that
$B_2 \in $ \gfgcfl,
yet Lemma~\ref{lem_not_DCFL} shows that its complement $B_2^c$
is not even a context-free language.
\end{proof}

\begin{lemma} \label{closure_difference}
\gfgcfl is not closed under set difference.
\end{lemma}
\begin{proof}
Closure under set difference implies closure under complementation since for every language $L$ over alphabet $\Sigma$, we have that the complement~$L^{c}$ is equal to $\Sigma^* \backslash L$.
\end{proof}

\begin{lemma} \label{closure_homomorphism}
\gfgcfl is not closed under homomorphism.
\end{lemma}
\begin{proof}
The language
\begin{align*}
L ={} &{}
\left\{
\,\binom{a}{1}^n \binom{b}{\#}^n 
\,\middle|\, n\geqslant 0 \, \right\} \, \cup \,
\left\{
\,\binom{a}{2}^n \binom{b}{\#}^{2n} 
\,\middle|\, n\geqslant 0 \, \right\}
\end{align*}
is recognised by a DPDA, and hence by an \HD-PDA using Lemma \ref{lemma_inclusions}, but its projection (which is a homomorphism)
\[ 
\set{ a^n b^n \mid n\geqslant 0} \cup \set{ a^n b^{2n} \mid n\geqslant 0}
\]
cannot be recognised by an \HD-PDA (see Lemma~\ref{lem:expressiveness1}). 
\end{proof}

\subsubsection{Closure Properties with Regular Languages}

\begin{theorem}
If $L$ is in \HD-CFL and $R$ is regular, then $L \cup R$, $L \cap R$ and $L \backslash R$ are also in \HD-CFL, but $R \backslash L$ is not necessarily in \HD-CFL.
\end{theorem}

\begin{proof}
Consider an \HD-PDA $\aut = (Q, \Sigma, \Gamma, q_\initmark, \Delta, F)$ recognising $L$, and a resolver~$\hstrat$ for $\aut$.
By definition, $\hstrat$ only has to induce a run on every $w \in L(\aut)$, but does not necessarily induce a run on $w \notin L(\aut)$. First, we turn $\aut$ into an equivalent \HD-PDA~$\aut'$ that has a resolver that induces a run on every input $w \in \Sigma^*$.
This property allows us then to take the product of $\aut'$ and an DFA for $R$.

To this end, we add a fresh nonfinal sink state~$q_s$ with a self-loop~$(q_s, X, a, q_s, X) $ for every input letter~$a\in \Sigma$ and every stack symbol~$X \in \Gammabot$. Also, we add transitions so that every configuration has, for every $a \in \Sigma$, an enabled $a$-transition to the sink. 
The resulting PDA~$\aut'$ is equivalent and $\hstrat$ is still a resolver for it. But, we can also turn $\hstrat$ into a resolver~$\hstrat'$ that induces a run on every possible input as follows:
If $\ell(\tau_0 \cdots \tau_n)$ is a prefix of a word in $L(\aut)$, then we define $\hstrat'(\tau_0 \cdots \tau_n, a) = \hstrat(\tau_0 \cdots \tau_n, a)$ for every $a \in \Sigma$. Otherwise, if $\ell(\tau_0 \cdots \tau_n)$ is not a prefix of a word in $L(\aut)$, we define $\hstrat'(\tau_0 \cdots \tau_n, a) = (q, X, a, q_s, X)$, where $(q, X)$ is the mode of the last configuration of the run induced by $\tau_0 \cdots \tau_n$. 
Thus, as soon as the input can no longer be extended to a word in $L(\aut)$, then run induced by $\hstrat'$ moves to the sink state and processes the remaining input. 

Now, let $\auta$ be a DFA recognising $R$.
For $L \cup R$, we construct the product~PDA~$\aut_\cup$ of $\aut'$ and $\auta$ that simulates a run of $\aut'$ and the unique run of $\auta$ simultaneously on an input word and accepts if either the run of $\aut$ or the run of $\auta$ is accepting.
We note that when an $\epsilon$-transition is chosen in $\aut'$ by the resolver, then no move is made in $\auta$. 
As $\aut'$ has a run on every input, the product PDA~$\aut_\cup$ has one as well.

For $L \cap R$, we construct a PDA $\aut_\cap$ which is similar to $\aut_\cup$ with the difference that $\aut_\cap$ accepts when each of $\aut'$ and $\auta$ has an accepting run on the input word.

Both $\aut_\cup$ and $\aut_\cap$ are \HD-PDA since only the nondeterminism of $\aut'$ needs to be resolved.

Finally, since $L\backslash R = L \cap R^c$ and the complement~$R^c$ is regular, it follows that $L \backslash R$ is recognised by an \HD-PDA if there is an \HD-PDA recognising $L$.
For $R \backslash L$, note that $\Sigma^*$ is a regular language and $\Sigma^*\backslash L = L^c$ which by Lemma \ref{closure_complementation} implies that $R \backslash L$ may not be in \HD-CFL.
\end{proof}

\subsubsection{Proof of Theorem~\ref{thm:expressiveness}}

We prove \dcfl $\subsetneq$ \gfgcfl $\subsetneq$ \cfl in several steps. Recall that we defined $
    B_2 = \{a^i \$ a^j \$ b^k \$ \mid k \leqslant \max(i,j)\}$.


\begin{lemma} \label{lem_expressiveness}
    $B_2 \in$ \gfgcfl.
\end{lemma}

\begin{proof}
Let us summarise the behaviour of the pushdown automaton $\aut_{B_2}$
recognising $B_2$ (see Figure \ref{fig:gfgpdaexample}).
First, the automaton copies the two blocks of $a$'s on
the stack.
Then, when it processes the second $\$$,
it transitions nondeterministically to either $p_1$ or $p_2$.
In $p_1$, it erases the second $a$-block from the stack,
so that the first block is at the top of the stack,
and then transitions to $p_2$.
In $p_2$, the automaton compares the number of $b$'s in the input
with the number of $a$'s in the topmost block of the stack.
If the latter is larger than or equal to the former,
$\aut_{B_2}$ pops one $a$ for each $b$ in the input,
and then transitions to the final state when it processes
the third $\$$.

When processing the second $\$$,
knowing whether the first or second block of the prefix contains more $a$'s
allows the nondeterminism to be resolved:
if the first block contains more $a$'s, take the transition to the state $p_1$,
if the second block contains more $a$'s, take the transition to the state $p_2$.
\end{proof}

To show that $B_2$ is not in $\dcfl$, we prove that its complement is not even context-free. This suffices, as $\dcfl$ is closed under complementation.

\begin{lemma} \label{lem_not_DCFL}
    The complement $B_2^c$ of $B_2$ is not in $\cfl$.
\end{lemma}

\begin{proof}
    Assume, for the sake of contradiction, that
    the complement $B_2^{c}$ of $B_2$ is in $\cfl$.
    Now consider the regular language
    \begin{align*}
    A &= \{a^i \$ a^j \$ b^k \$| i,j,k \in \mathbb{N}\}.
    \end{align*}
    Since the intersection of a context-free language and a regular language is context-free,
    we have that $B_2^{c}\cap A \in \cfl$.
    Therefore, $B_2^{c} \cap A$ satisfies the pumping lemma for context-free languages:
    there exists $m \in \mathbb{N}$ such that the word $z = a^m \$ a^m \$ b^{m+1}\$ \in B_2^{c} \cap A$
    can be decomposed as $z = uvwxy$ such that
    \begin{enumerate}
        \item\label{item:pump_empty} $|vx| \geqslant 1$;
        \item\label{item:pump_iter} $uv^nwx^ny \in B_2^{c}\cap A$ for every $n \geqslant 0$.
    \end{enumerate}
    Note that Item \ref{item:pump_iter} directly implies that both $v$ and $x$ are in the language
    $\{a\}^* \cup \{b\}^*$,
    as otherwise $uv^2wx^2y$ is not in $A$.
    On top of that, Item~\ref{item:pump_empty} implies that either $v$ or $x$ is in
    $\{a\}^+ \cup \{b\}^+ $.
    We conclude by proving, through a case distinction, that Item~\ref{item:pump_iter}
    cannot hold as either $uwy$ or $uv^2wx^2y$ is in $B_2$.
    \begin{itemize}
        \item
        Assume that neither $v$ nor $x$ is in $\{b\}^+$.
        Then either $v$ or $x$ is in $\{a\}^+$,
        hence $uv^2wx^2y= a^{m_1} \$ a^{m_2} \$ b^{m+1}\$$ for some $m_1,m_2 \geqslant m$
        such that either $m_1>m$ or $m_2>m$.
        In both cases, we get $uv^2wx^2y \in B_2$.
        \item
        Assume that either $v$ or $x$ is in $\{b\}^+$.
        Then pumping $v$ and $x$ down in $z$ reduces the size
        of at most one of the $a$-blocks:
        we have that $uwy = a^{m_1} \$ a^{m_2} \$ b^{m_3 +1}\$$
        for $m_1,m_2,m_3 \leqslant m$ such that $m_3<m$, and either $m_1 = m$ or $m_2 = m$.
        In both cases, we get $uwy \in B_2$.
    \end{itemize}
    As every possible case results in a contradiction, 
    our initial hypothesis is false:
    $B_2^c \not\in$ \cfl.
\end{proof}

The previous two lemmata and Lemma~\ref{lemma_inclusions} yield \dcfl $\subsetneq$ \gfgcfl.

Now, we prove \gfgcfl $\subsetneq$ \cfl. Recall that we defined $L = \{a^nb^n  \mid  n \geqslant 0\} \cup \{a^nb^{2n}  \mid  n \geqslant 0\}$, which is clearly in \cfl. Hence, the following lemma completes the proof of Theorem~\ref{thm:expressiveness}.

\begin{lemma} \label{lem:expressiveness1}
$L \notin $ \gfgcfl.
\end{lemma}

\begin{proof}
We show that there does not exist an \HD-PDA recognising $L$.
In fact, we show that if there existed an \HD-PDA $\aut$ recognising $L$, then we could construct a PDA $\widehat{\aut}$ recognising the language $\widehat{L}=L \cup \{a^n b^n c^n  \mid  n \geqslant 0\}$.
Since $\widehat{L}$ is not in \cfl, we would thus reach a contradiction.

The idea behind the construction is to replicate the part of the control unit of $\aut$ which processes the suffix $b^n$ of an input word $a^nb^{2n}$ with the difference that in the newly added parts, the transitions caused by input symbol $b$ are replaced with similar ones for input symbol $c$.
This new part of the control unit may be entered after $\widehat{\aut}$ has processed $a^nb^n$.

We now construct the PDA $\widehat{\aut}$ from $\aut$ as follows.
Let $\aut = (Q, \Sigma, \Gamma, q_I, \Delta, F)$ with $Q=\{q_0, q_1, \dots, q_n\}$, and let $q_0=q_\initmark$.
Now consider $\widehat{\aut} = (Q \cup \widehat{Q}, \Sigma, \Gamma, q_I, \Delta \cup \widehat{\Delta}, F \cup \widehat{F})$ with
$\widehat{Q} =\{\widehat{q}_0, \widehat{q}_1, \dots, \widehat{q}_n\}$, $\widehat{F} =\{\widehat{q_i}  \mid  q_i \in F\}$,
and $\widehat{\Delta}$ includes the following additional transitions:
\begin{enumerate}[1.]
    \item $\{(q_f, X, \epsilon, \widehat{q}_f, X) \mid q_f \in F, X \in \Gammabot\}$: switch from the original final states to the new states.
    \item $\{(\widehat{q}_i, X, c, \widehat{q}_j, \gamma) \mid (q_i, X, b, q_j, \gamma) \in \Delta \}$: replicate the original $b$-transitions by $c$-transitions in the new states.
    \item \{$(\widehat{q}_i, X, \epsilon, \widehat{q}_j, \gamma) \mid (q_i, X, \epsilon, q_j, \gamma) \in \Delta \}$: replicate all $\epsilon$-transitions. 
\end{enumerate}

Now we show that $L(\widehat{\aut})=\widehat{L}$.
First we show that $L(\widehat{\aut}) \subseteq \widehat{L}$.
Consider a word $w \in L(\widehat{\aut})$.
There may be two cases:
\begin{enumerate}[(i)]
    \item Assume $\widehat{\aut}$ has an accepting run on $w$ that does not visit a state in $\widehat{Q}$. In this case, we have that $w$ is in $L(\aut)=L\subseteq \widehat{L}$.
    
    \item Assume there exists an accepting run of $\widehat{\aut}$ on $w$ that visits a state in $\widehat{Q}$.
    Since $\aut$ recognises $L$, and by construction of $\widehat{\aut}$, a state $\widehat{q}_i \in \widehat{Q}$ can be reached from a state $q_i \in Q$ only if $\widehat{q}_i \in \widehat{F}$ and $q_i \in F$, and the corresponding transition is an $\epsilon$-transition, we have that starting from the initial configuration $(q_\initmark, \bot)$, a state in $\widehat{Q}$ is reached for the first time only after processing an input prefix $a^nb^n$ or $a^nb^{2n}$ for some $n \geqslant 0$.
    If this prefix of $w$ is $a^nb^{2n}$, then $w=a^nb^{2n}$.
    This is because if $w=a^nb^{2n}c^m$ for some $m > 0$ (recall that after visiting a state $\widehat{q}_i$ in $\widehat{Q}$, the only non-$\epsilon$ transitions possible are on the letter $c$), then by the construction of $\widehat{\aut}$, we have that $\aut$ can accept the word $a^nb^{2n}b^m$ which is not in the language $L$.
    On the other hand, let the prefix be $a^nb^n$ when a state $\widehat{q}_i \in \widehat{Q}$ is visited for the first time.
    Note that $\widehat{q}_i \in \widehat{F}$, and  let $(\widehat{q}_i, \gamma_i)$ be the corresponding configuration.
    If a sequence of transitions $\widehat{\tau}_i \dots \widehat{\tau}_j$ from $(\widehat{q}_i, \gamma_i)$ to $(\widehat{q}_j, \gamma_j)$ is possible such that not all of $\widehat{\tau_i} \dots \widehat{\tau_j}$ are $\epsilon$-transitions, that is, the transitions process $c^m$ for some $m \in \nats$, and $\widehat{q}_j \in \widehat{F}$, then a sequence of transitions $\tau_i \dots \tau_j$ of the same length processing $b^m$ is possible from $(q_i, \gamma_i)$ to $(q_j, \gamma_j)$ with $q_j \in F$.
    Since this leads to an accepting run from $(q_\initmark, \bot)$ to $(q_j, \gamma_j)$ while visiting only the states in $Q$ on processing $a^nb^nb^m$ with $m > 0$, we have $m=n$, and hence $w=a^nb^nc^n \in \widehat{L}$.
    
    If on the other hand, if all the transitions $\widehat{\tau_i} \dots \widehat{\tau_j}$ are $\epsilon$-transitions, then $w=a^nb^n \in \widehat{L}$.
\end{enumerate}

Now we prove the other direction, that is $\widehat{L} \subseteq L(\widehat{\aut})$.
Here, we rely on the fact that the accepting run of $\aut$ on $a^nb^n$ induced by $\hstrat$ is a prefix of the accepting run of $\aut$ on $a^nb^{2n}$ induced by $\hstrat$. This allows to switch to the copied states~$\widehat{Q}$ after processing $a^nb^n$ and then process $c^n$ instead of $b^n$.

Consider a word $w \in \widehat{L}$ such that $w \in L$.
By construction of $\widehat{\aut}$, we have that $w \in L(\widehat{\aut})$ since $\widehat{\aut}$ accepts all words that are also accepted by $\aut$.
Now suppose that $w \in \widehat{L}$ but $w \notin L$, that is, $w$ is of the form $a^nb^nc^n$ for some $n \geqslant 1$.
Since by assumption, we have that $\aut$ is an \HD-PDA recognising the language $L$, there exists a resolver $r$ that for every word in $L$ induces an accepting run of the word in $L$.
Let  $(q_i, \gamma_i)$ be  the configuration of $\aut$ reached after processing the prefix $a^nb^n$ in the run induced by $r$ on the input $a^nb^{2n}$. 

Note that $q_i \in F$ since $r$ also induces an accepting run for the input $a^nb^n$.
Now if for the input $a^nb^{2n}$, the sequence of transitions chosen by $r$ from $(q_i, \gamma_i)$ after processing $a^nb^n$ is $\tau_i, \tau_{i+1}, \cdots, \tau_j$ with $(q_i, \gamma_i) \trans{\tau_{i}} (q_{i+1}, \gamma_{i+1}) \dots (q_{j-1}, \gamma_{j-1}) \trans{\tau_j} (q_j,\gamma_j)$, with $q_j \in F$, and the sequence $\tau_i, \dots, \tau_j$ processes $b^n$, then by the construction of $\widehat{\aut}$, there exists a sequence of transitions $\widehat{\tau}_{i}, \widehat{\tau}_{i+1}, \dots, \widehat{\tau}_j$ with $(\widehat{q}_i, \gamma_i) \trans{\widehat{\tau}_i} (\widehat{q}_{i+1}, \gamma_{i+1}) \dots (\widehat{q}_{j-1}, \gamma_{j-1}) \trans{\widehat{\tau}_j} (\widehat{q}_j, \gamma_j)$ and with $\widehat{q}_j \in \widehat{F}$ such that there is an $\epsilon$-transition from $(q_i, \gamma_i)$ to $(\widehat{q}_{i}, \gamma_{i})$ and the sequence $\widehat{\tau}_i, \widehat{\tau}_{i+1}, \cdots, \widehat{\tau}_j$ processes $c^n$, and hence $w \in L(\widehat{\aut})$.

Thus we have that $\widehat{L}=L(\widehat{\aut})$.
Hence we show that if $\aut$ is an \HD-PDA, then we can construct a PDA $\widehat{\aut}$ recognising $\widehat{L}$ which is not a CFL, thus leading to a contradiction to our assumption that $L$ is in \HD-CFL.
\end{proof}

\subsubsection{Proof of Theorem~\ref{unamb_vs_gfg}} 
\label{app:ambiguity}
We need to show that $B=\{a^i b^j c^k \mid i,j,k \geqslant 1, k \leqslant \max(i,j)\}$ is inherently ambiguous, i.e.\ for every grammar generating $B$ there is at least one word that has two different leftmost derivations.

We use standard definitions and notation for context-free grammars as in~\cite{Hopcroft}. We say that a grammar is reduced, if every variable is reachable from the start variable, every variable can be reduced to a word of terminals, and for no variable $A$, it holds that $A {\overset{*}{\implies}}A$.


Let $D(G) = \{A \in V \mid A  {\overset{*}{\implies}} x A y \text{ for some } x,y \text{ with } xy\neq \epsilon\}$.
An unambiguous CFG $G$ is called \emph{almost-looping}, if
\begin{enumerate}
    \item $G$ is reduced,
    \item all variables, possibly other than the start variable $S$, belong to $D(G)$, and
    \item either $S \in D(G)$ or $S$ occurs only once in the leftmost derivation of any word in $L(G)$.
\end{enumerate}

Now we state the following lemma from \cite{Maurer69}.
\begin{lemma} \label{lem:Maurer}
For every unambiguous CFG $G$, there exists an unambiguous almost-looping CFG $G'$ such that $L(G)=L(G')$.
\end{lemma}

An important property of the grammar obtained through the translation is that if the initial grammar is unambiguous, then so is the translated almost-looping grammar.

An example of an almost-looping grammar for language $B$ is the following:
\begin{figure}[h]
% \centering
\begin{minipage}{0.4\textwidth}
% \centering
$S \rightarrow S_1  \mid  S_2$ \\
$S_1 \rightarrow aS_1  \mid  aS_1c  \mid  aBc$\\
$B \rightarrow bB  \mid  b$\\
\end{minipage}
\begin{minipage}{0.4\textwidth}
% \centering
$S_2 \rightarrow aS_2  \mid  aD$\\
$D \rightarrow bDc  \mid  bD  \mid  bc$\\
\end{minipage}
\centering
\caption{An example CFG for language $B$}
\label{fig:cfg1}
\end{figure}

Now we prove the following, using techniques inspired by Maurer's proof that $\set{a^i b^j c^ k \mid i,j,k \geqslant 1, i=j \vee j=k}$ is inherently ambiguous~\cite{Maurer69}.

\begin{lemma}
The language $B$ is inherently ambiguous.
\end{lemma}

\begin{proof}
Assume, towards a contradiction, that $G$ is an unambiguous grammar for $B$, which, from Lemma~\ref{lem:Maurer}, we can assume, without loss of generality, to be an almost-looping grammar.
Let $A$ be a variable of $G$.
\begin{enumerate}
    
    \item \label{onlya} $A$ is of Type~\ref{onlya} if there is a derivation~$A {\overset{*}{\implies}} xAy$ where $xy=a^{\markingn{A}{1}}$ for some $\markingn{A}{1} > 0$.

    \item \label{onlyb} $A$ is of Type~\ref{onlyb} if there is a derivation~$A {\overset{*}{\implies}} xAy$ where $xy=b^{\markingn{A}{2}}$ for some $\markingn{A}{2} > 0$.
    
    \item \label{ac} $A$ is of Type~\ref{ac} if there is a derivation~$A {\overset{*}{\implies}} xAy$ where $x=a^{\markingl{A}{3}}$ and $y=c^{\markingr{A}{3}}$ for some $\markingl{A}{3} \geqslant \markingr{A}{3} > 0$.
    
    \item \label{bc} $A$ is of Type~\ref{bc} if there is a derivation~$A {\overset{*}{\implies}} xAy$ where $x=b^{\markingl{A}{4}}$ and $y=c^{\markingr{A}{4}}$ for some $\markingl{A}{4} \geqslant \markingr{A}{4} > 0$.
    
    \item \label{ab} $A$ is of Type~\ref{ab} if there is a derivation~$A {\overset{*}{\implies}} xAy$ where $x=a^{\markingl{A}{5}}$ and $y=b^{\markingr{A}{5}}$ for some $\markingl{A}{5}, \markingr{A}{5} > 0$.    
\end{enumerate}
Note that some variables may be of multiple types (e.g.\ the variable~$D$ in Figure~\ref{fig:cfg1}
 has Type~\ref{onlyb} and Type~\ref{bc}).
s
First, we show that each variable in $D(G)$ has at least one of these five types.
So, let $A \in D(G)$. Then, there exists a derivation~$A {\overset{*}{\implies}} xAy$ with $xy\neq\epsilon$.
Note that both $x$ and $y$ belong to $a^*$, $b^*$, or $c^*$ since otherwise, due to $G$ being reduced, one could derive words that are not in the language.
Next, we note that the cases where $x$ belongs to $c^*$, and $y$ belongs to $a^*$ or $b^*$ cannot happen.
Similarly, the case where $x$ belongs to $b^*$, and $y$ belongs to $a^*$ cannot happen.
Also we cannot have $xy$ in $c^*$, since this will allow us to have words with arbitrary number of $c$'s which can be more than the number of $a$'s and $b$'s and such a word is not in the language.

Further, we cannot have $x=a^{\ell}$ and $y=c^{r}$ with $0 < \ell < r$. Otherwise, consider a derivation of some word in $B$ that uses $A$, i.e.\ \[S {\overset{*}{\implies}} \alpha A \beta {\overset{*}{\implies}} a^s b^u c^v \text{\quad with $v \leqslant \max(s,u)$.}\]  Now, towards a contradiction assume we indeed have \[A {\overset{*}{\implies}} x A y \text{\quad with $x=a^{\ell}, y=c^{r}$ and $\ell < r$.}\] 
Then, pumping $q$ copies of $x$ and $y$, for some suitable $q \in\nats$, yields a derivation
\[
S {\overset{*}{\implies}} \alpha A \beta {\overset{*}{\implies}} \alpha x^q A y^q \beta {\overset{*}{\implies}} a^{s+\ell q} b^{u} c^{v+r q}
\text{\quad such that $v+rq > \max(s+\ell q, u)$},
\]
i.e.\ we have derived a word that is not in $B$.
Similarly, we cannot have $x=b^\ell$ and $y=c^r$ for some $0 < \ell < r$.
Altogether, this implies that $A$ indeed has at least one of the five types stated above.


Moreover, we claim that there is a $t \in \nats$ such that the following three properties are true for every word~$w \in B$:
\begin{description}
    \item[Property 1] If $w$ has more than $t$ $c$'s, then the (unique) leftmost derivation of $w$ has the form  
    \[S {\overset{*}{\implies}} \alpha A \beta {\overset{*}{\implies}} \alpha x A y \beta {\overset{*}{\implies}} w
    \text{\quad such that $xy$ contains a $c$. }\]
    Thus, $A$ has type~\ref{ac} or type~\ref{bc}.

\item [Property 2] If $w$ has more than $t$ $a$'s, then the (unique) leftmost derivation of $w$ has the form  
    \[S {\overset{*}{\implies}} \alpha A \beta {\overset{*}{\implies}} \alpha x A y \beta {\overset{*}{\implies}} w
    \text{\quad such that $xy$ contains an $a$. }\]
    Thus, $A$ has type~\ref{onlya}, type~\ref{ac}, or type~\ref{ab}.
    
\item [Property 3] If $w$ has more than $t$ $b$'s, then the (unique) leftmost derivation of $w$ has the form  
    \[S {\overset{*}{\implies}} \alpha A \beta {\overset{*}{\implies}} \alpha x A y \beta {\overset{*}{\implies}} w
    \text{\quad such that $xy$ contains a $b$. }\]
    Thus, $A$ has type~\ref{onlyb}, type~\ref{bc}, or type~\ref{ab}.
\end{description}

We prove these properties as follows:
we denote by $d$ the \emph{width} of the grammar $G$
which is the maximum number of symbols appearing on the right side of some production rule of $G$.
Further, we denote by $m$ the number of variables appearing in $G$.
We argue that $t = d^{m+1}$ satisfies the three properties above.
We focus on Property~1, the two other proofs are similar.
Suppose that $w$ contains more than $d^{m+1}$ $c$'s and consider the derivation tree of that word.
The \emph{weight}~$\omega(v)$ of a vertex~$v$ in the derivation tree is defined as the number of $c$'s in the subtree rooted at~$v$.
Hence, the root of the derivation tree has at least weight~$d^{m+1}$.
We build a finite path $v_0,v_1, \ldots, v_k$
from the root of this tree to one of its leaves as follows:
The initial vertex~$v_0$ is the root and
at each step, we choose as successor of $v_{i}$
its child $v_{i+1}$ with the largest weight.
A vertex~$v_{i}$ of this path is \emph{decreasing} if $\omega(v_{i}) > \omega(v_{i+1})$.
There are are at least $m+1$ decreasing vertices on the path
because 
$\omega(v_0) = d^{m+1}$,
$\omega(v_k) = 1$,
and $\omega(v_{i+1}) \geq \frac{1}{d} \cdot \omega(v_i)$.
Thus, there are two decreasing vertices on the path that are labeled by the same variable~$A$ such that there is a derivation of the form~$A {\overset{*}{\implies}} xAy$ with some $c$ in $xy$.

Let $p > t$ be a positive integer divisible by the least common multiple of the $\markingn{A}{i}, \markingl{A}{i}$ and $\markingr{A}{i}$ for all $A \in D(G)$ and $i \in \set{1, \ldots, 5}$, where we define $\markingn{A}{1} = 1$ if $A$ is not of Type~\ref{onlya}, and similarly for all other~$i > 1$.
We show that the word $w = a^{2p}b^{2p}c^{2p} \in B$ has two leftmost derivations.

First consider the derivation of the word $w_b = a^{2p}b^{p}c^{2p} \in B$.
As we have more than $t$ $c$'s in $w_b$ Property~1 shows that the derivation contains a variable of Type~\ref{ac} or Type~\ref{bc}. 
Next, we argue that it cannot contain a variable of Type~\ref{bc}: The occurrence of such a variable would allow us to either produce a word that is not in $a^*b^*c^*$ or to inject $b^{p}c^{r}$ for $p \geqslant r > 0$ leading to the derivation of $a^{2p}b^{2p}c^{2p+r}$, which is not in the language.
Thus, the derivation of $w_b$  uses at least one variable of Type~\ref{ac}.
Also, since $w_b$ has $p > t$ $b$'s,
Property~3 implies that the (unique) leftmost derivation of $w_b$ has the form
\[S {\overset{*}{\implies}} \alpha A \beta {\overset{*}{\implies}} \alpha x A y \beta {\overset{*}{\implies}} w_b
    \text{\quad such that $xy$ contains a $b$. }\]
Thus $A$ is a variable of Type~\ref{onlyb} or Type~\ref{ab}
(note that we have already ruled out Type~\ref{bc} above).
More precisely, we have that $x$ belongs to $a^+$ or $b^*$ and $y = b^j$ for some $j \in \nats$.
Now we show that the case where $x$ belongs to $a^+$ is not possible.
Assume for contradiction that $x = a^i$ for some $i>0$.
Then we also have the derivation
\[S {\overset{*}{\implies}} \alpha A \beta {\overset{*}{\implies}} a^{2p-i}b^{p-j}c^{2p} \notin B.\]
Therefore, $A$ is a Type~\ref{onlyb} variable that is used in the derivation of $w_b$, which can be used to inject another $b^p$, yielding a derivation of $w$. Thus, we have exhibited a derivation of $w$ that uses a variable of Type~\ref{ac}.


Now consider a derivation of the word $w_a = a^{p}b^{2p}c^{2p}$.
Such a derivation cannot contain a variable of Type~\ref{ac} since this allows us either to produce a word that is not in $a^*b^*c^*$ or to inject $a^{p}c^{r}$ for $p \geqslant r > 0$, leading to the derivation of $a^{2p}b^{2p}c^{2p+r} \notin B$.
Further, arguing as above, some variable of Type~\ref{onlya}
must appear in the derivation of $w_a$ that is used to obtain sufficient number of $a$'s in the derivation of $w_a$.
Such a variable of Type~\ref{onlya} can be used to inject $a^p$ into $w_a$ which leads to the derivation of $w$.
Thus, we have exhibited a derivation of $w$ that does not contain a variable of Type~\ref{ac}.

Altogether, there are two different leftmost derivations of the word $w$.
Thus, $G$ is not unambiguous, yielding the desired contradiction.
\end{proof}

\subsubsection{Proof of Theorem~\ref{theorem:succinctness}}

Recall that we need to prove that \HD-PDA can be exponentially more succinct than DPDA,
and that PDA can be
double-exponentially more succinct than \HD-PDA.

We first consider the gap between DPDA and \HD-PDA.
Recall that we defined $c_n\in (\$\{0,1\}^n)^*$ to be the word describing
an $n$-bit binary counter counting from $0$ to $2^{n}-1$ and 
\[
C_n= \big\{w \in \{0,1,\$,\#\}^*| w \neq c_n\#\big\}.
\]
We prove that $C_n$ is recognised by a PDA of linear size, but every \HD-PDA recognising $C_n$ has exponential size. The proof is split into two parts.

\begin{lemma}
\label{lemma:succinct_GFGPDA1}
The language $C_n$ is recognised by
an \gfgpda{} of size $O(n)$.
\end{lemma}

\begin{proof}
We define a PDA~$\aut=(Q, \Sigma, \Gamma, q_\initmark, \Delta, F)$ that recognises $C_n$.
The automaton $\aut$
operates in three phases:
a push phase,
followed by a check phase,
and then a final phase.
These phases work as follows.
Suppose that $\aut$ receives an input $w \in \{0,1,\$,\#\}^*$.
During the first phase, $\aut$ pushes the input processed onto the stack until the sequence $1^n$ appears.
If it never appears, the input is accepted.
During this phase, $\aut$ also checks whether the prefix $w'$ of $w$
processed up to this point
is a sequence of counter values starting with $0^n$,
i.e. whether $w'$ is in the language
\[
L_c=
\{
\$d_0\$ d_1\$ \cdots \$ d_m \mid
 d_0 = 0^n,
 d_i = 1^n \Leftrightarrow i = m,
\textup{ and }
 d_i \in \{0,1\}^n
 \textup{ for all }
 1 \leqslant i \leqslant m
 \}.
\]
If $w' \not\in L_c$,
then $\aut$ immediately accepts.
Otherwise, $\aut$ moves to the second phase.
During the check phase, $\aut$ pops the stack.
At any point, $\aut$ can nondeterministically guess that the top symbol of the stack
is evidence of bad counting. It then accepts the input if the guess was correct.
If $\aut$ completely pops the stack without
correctly guessing an error in the counter,
it moves to the final phase.
Since the prefix $w'$ processed up to this point
ends with the sequence $1^n$,
if $\aut$ now processes any suffix different from a single $\#$,
then the input is not equal to $c_n\#$, and can be accepted.

The stack alphabet of $\aut$ has constant size $3$.
The push phase requires $3(n+1)$ states:
\begin{itemize}
    \item First, $\aut$ checks whether $\$ 0^n$ is a prefix of the input.
    This can be done with $n + 2$ states.
    \item Then, $\aut$ checks whether the following $\{0,1\}^*$ segments are $n$-bits wide,
    and only the last one is $1^n$.
    This can be done with $2n+1$ additional states:
    repeatedly, $\aut$ processes $n+1$ symbols,
    checks whether only the first of them is a $\$$,
    and keeps track of whether at least one of them is $0$.
\end{itemize}

We now show that $6(n+1)$ additional states
are enough for the check phase.
To this end, we study the errors that $\aut$ needs to check.
Note that, to increment the counter correctly,
we need to change the value of all the bits starting from the last $0$,
and leave the previous bits unchanged.
Therefore, $\aut$ can recognise with $6(n+1)$ states
whether the top symbol of the stack does not correspond
to a correct counter increment:
$\aut$ pops the top $n+1$ stack symbols while keeping in memory
\begin{itemize}
    \item the value of the first symbol popped;
    \item whether we have not yet popped a $\$$ (there is exactly one $\$$ in the top $n+1$ stack symbols, as the stack content is in $L_c$),
    or a $\$$ but no $0$ afterwards,
    or a $\$$ and at least one $0$ afterwards.
\end{itemize}
The input is accepted whenever the first symbol popped and the top stack symbol after popping match
yet no $0$ has been popped between the $\$$ and the last symbol,
or they differ yet at least one $0$ has been popped
between the $\$$ and the last symbol.

Finally, only three states are needed for the final phase:
when the bottom of the stack is reached, $\aut$
transitions to a new state, and from there it checks
whether the suffix is in the language
$\{0,1,\$,\# \}^* \setminus \{ \# \}$.


To conclude, note that $\aut$ is history-deterministic:
the only nondeterministic choice happens during the check phase,
and the resolver knows which symbols of the stack are evidence of bad counting.
Note that this choice only depends
on the current stack content.
\end{proof}

\begin{lemma}
\label{lemma:succinct_GFGPDA2}
Every DPDA recognising the language $C_n$ has
at least exponential size in $n$.
\end{lemma}

\begin{proof}
It is known that every DPDA can be complemented
at the cost of multiplying
its number of states by three~\cite{Hopcroft}.
Therefore, to prove the statement,
we show that even every PDA recognising 
the complement $\{c_n\#\}$ of $C_n$
has at least exponential size in $n$:

\begin{claim}
Every PDA $\aut=(Q, \Sigma, \Gamma, q_\initmark, \Delta, F)$
recognising $\{ c_n\# \}$ has a size greater than $2^{(n-1)/3}$.
\end{claim}
To prove the claim, we transform $\aut$ into a context-free
grammar generating the singleton language $\{ c_n\# \}$,
and then we show that such a grammar requires
exponentially many variables.
This is a direct consequence of the $mk$ Lemma~\cite{DBLP:journals/tit/CharikarLLPPSS05},
but proving it directly using similar techniques yields a slightly better bound.

Before changing $\aut$ into a grammar,
we slightly modify
its acceptance condition:
we add to $\aut$ a fresh final state $f$
in which the stack can be completely popped
\emph{including the bottom of stack symbol} $\bot$
(which normally cannot be touched
according to our definition of PDA).
Moreover, we allow $\aut$ to transition
towards $f$ nondeterministically
from all of its other final states.
This new automaton, which accepts by empty stack,
is easily transformed into 
a grammar $\mathcal{G}$ using
the standard transformation~\cite{Hopcroft}:
\begin{itemize}
    \item The terminals of $\mathcal{G}$ are $0$, $1$, $\$$ and $\#$.
    \item The variables of $\mathcal{G}$ are the triples $(p,X,q)$,
    for every state $p, q \in Q \cup \{f\}$ and stack symbol
    $X \in \Gamma_{\bot}$.
    \item The initial variable is $(q_\initmark, \bot, f)$,
    where $q_\initmark$ is the initial state of $\aut$
    and $f$ is the fresh final state.
    \item
    Each transition $(p,X,a,q,\gamma) \in \Delta$ yields production rules as follows:
    \begin{enumerate}\item
        If $\gamma = \epsilon$, then $\mathcal{G}$
        has the production rule
        $(p,X,q) \rightarrow a$;
        \item
        If $\gamma = Y$,
        then
        $\mathcal{G}$ has the production rule $(p,X,q_1) \rightarrow a (q,Y,q_1)$
        for all $q_1 \in Q$;
        \item 
        If $\gamma = YZ$,
        then
        $\mathcal{G}$ has the production rule
        $(p,X,q_2) \rightarrow a (q,Y,q_1) (q_1,Z,q_2)$
        for all $q_1,q_2 \in Q$.
    \end{enumerate}
\end{itemize}
The variables can be interpreted as follows:
for every $p, q \in Q$ and $X \in \Gamma$,
the variable $(p,X,q)$ can be derived into any input word $w \in \{0,1,\$\}^*$
that $\aut$ can process starting in state $p$ and ending in state $q$
while consuming the symbol $X$ from the top of the stack.
Therefore, in particular, 
since the initial variable is $(q_\initmark, \bot, f)$,
$\mathcal{G}$ generates the same language as $\aut$.


We now prove that the grammar $\mathcal{G}$
has at least $2^{n-1}$ distinct variables,
hence $(|Q|+1)^2(|\Gamma|+1) \geqslant 2^{n-1}$,
which implies that the size
$|Q| + |\Gamma|$ of $\aut$ is at least $\geqslant 2^{(n-1)/3}$.
To this end, we study a (directed) derivation tree $T$ of the word $c_n\#$.


Remember that $c_n = \$d_0\$d_1\$ \cdots \$ d_{2^{n}-1}$ represents
an $n$-bit binary counter counting from $0$ to $2^n-1$.
For each $0 \leq i \leq 2^n-1$,
let us consider the vertex $v_i$ of $T$
such that the counter value $d_i$ is an infix of the derivation of $v_i$,
but of none of its children.
In other words, $d_i$ is split between the derivations of the children of $v_i$.
By definition of the grammar $\mathcal{G}$,
each vertex of $T$ has at most three children,
hence at most two counter values can be split amongst the children of a given vertex, 
which implies that $v_i \neq v_{i+2}$ for all $0 \leq i \leq 2^{n-3}$.
Therefore, the vertices $v_0,v_2,v_4, \ldots, v_{2^n-2}$ are all distinct.
Finally, since $c_n\#$ is the only word recognised by $\aut$
and each counter value $d \in \{0,1\}^n$ appears a single time as an infix of $c_n\#$,
the $2^{n-1}$ variables labelling these vertices need to be distinct.
\end{proof}


Now, we consider the gap between \HD-PDA and PDA.
Recall that $L_n$ is the language of words over $\set{0,1}$ such that the $n^{\text{th}}$ bit from the end is a $1$. We need to show that there exists a PDA of size $O(\log n)$ recognising $L_n$, and that every \HD-PDA recognizing $L_n$ has exponential size. Again, the proof is split into two parts.

\begin{lemma}
\label{lem:PDA-logn}
There exists a PDA of size $O(\log n)$ recognising $L_n$.
\end{lemma}

\begin{proof}
We describe a PDA $\aut$ that recognises $L_n$.
The PDA $\aut$ nondeterministically guesses the $n^\text{th}$ bit from the end, checks that it is a $1$ and switches to a counting gadget that checks that the word ends in $n$ steps, as follows:
\begin{enumerate}[(i)]
    \item It pushes the binary representation of $n-2$ onto the stack.
    For example, if $n=8$, then $110$ is pushed onto the stack with $0$ at the top.
    Note that $\log (n-2)$ states suffice for pushing the binary representation of $n-2$.
    If $n=1$, then instead of pushing anything onto the stack, the automaton directly moves to a final state without any enabled transitions.
    \item \label{step:counter} Then $\aut$ moves to a state that attempts to decrement the counter by one for each successive input letter, as follows:
    When an input letter is processed, it pops $m$ $0$'s until $1$ is at the top of the stack, replaces the $1$ with a $0$, and finally pushes $m$ $1$'s back onto the stack before processing the next letter.
     If the stack empties before a $1$ is at the top of the stack, then the counter value is $0$ and the automaton moves to  a final state with no enabled transitions.
    Note that $O(\log n)$ states again suffice for this step.
\end{enumerate}
Thus $\aut$ has $O(\log n)$ states.
Note that for all $n$, $\aut$ uses only three stack symbols that are 0, 1, and $\bot$.
Thus the size of $\aut$ is $O(\log n)$, and $\aut$ recognises $L_n$.
\end{proof}

\begin{lemma}
\label{lem:GFG-PDA-exponential}
Every \HD-PDA recognising $L_n$ has at least exponential size in $n$.
\end{lemma}

 Towards proving this, we define the following notions.
We say that a word $w$ of length $n$ is \emph{rotationally equivalent} to a word $w'$ if $w'$ is obtained from $w$ by rotating it.
For example, the word $w=1101$ is rotationally equivalent to  $w'=1110$ since $w'$ can be obtained from $w$ by rotating it once to the right.
Note that the words that are rotationally equivalent form an equivalence class, and thus rotational equivalence partitions $\{0,1\}^n$.
Since the size of each class is at most $n$, the number of equivalence classes is at least $\frac{2^n}{n}$.

Now, we define the \emph{stack height} of a configuration~$c= (q, \gamma)$ as $\sh(c) = \size{\gamma}-1$,
and we define \emph{steps} of a run as usual:
Consider a run~$c_0 \tau_0 c_1 \tau_1 \cdots c_{n-1} \tau_{n-1} c_n$.
A position $s$ is a step if for all $s' \geqslant s$, we have that $\sh(c_{s'})\geqslant \sh(c_s)$, that is, the stack height is always at least $\sh(c_s)$ after position $s$.
Any infinite run of a PDA has infinitely many steps.
We have the following observation.
\begin{proposition} \label{prop:steps}
If two runs of a PDA have steps $s_0$ and $s_1$, respectively, with the same mode, then the suffix of the run following the step $s_0$ can replace the suffix of the other run following the step $s_1$, and the resultant run is a valid run of the PDA.
\end{proposition}

Now, we are ready to prove Lemma~\ref{lem:GFG-PDA-exponential}. Here, we work with infinite inputs for \HD-PDA. The run induced by a resolver on such an input is the limit of the runs on the prefixes.

\begin{proof}
Let $\aut$ be an \HD-PDA with resolver~$r$ that recognises $L_n$ with a set~$Q$ of states and a stack alphabet~$\Gamma$. We show that $|Q| \cdot |\Gamma| \geqslant \frac{2^n}{n}$.

Towards a contradiction, assume that $|Q|\cdot |\Gamma| < \frac{2^n}{n}$.
Then there exist two words $w_0$ and $w_1$ of length~$n$ that are not rotationally equivalent and such that the runs~$\rho_0$ and $\rho_1$ of $\aut$ induced by $\hstrat$ on $w_0^\omega$ and $w_1^\omega$ contain steps with the same mode, at positions $s_0$ and $s_1$ in $\rho_0$ and $\rho_1$ respectively, such that at least $n$ letters are processed  before $s_0$ and $s_1$.
Now consider in each of these two runs the sequence of input letters of length $n$
preceding and including the step position.
Let these $n$ letter words be $w_0'$ and $w_1'$ respectively.
Since $w_0$ and $w_1$ are not rotationally equivalent, $w_0'$ and $w_1'$ differ in at least one position $j \leqslant n$.

W.l.o.g., assume that for $w_0'$, the bit at position $j$ is $0$, while it is $1$ at position $j$ for $w_1'$.
Since the resolver chooses a run such that for every word where the $n^\text{th}$ letter from the end is a $1$ is accepted, this implies that $\rho_0$ does not visit a final state after processing $j-1$ letters after $s_0$, while $\rho_1$ visits a final state after processing $j-1$ letters after $s_1$.

Now we reach a contradiction as follows.
The suffix of $\rho_0$ starting from position $s_0+1$ can be replaced with the suffix of $\rho_1$ starting from position $s_1+1$. 
By Proposition~\ref{prop:steps}, this yields a valid run~$\rho$ of $\aut$.
However, since the state that occurs after $j-1$ letters are processed after position $s_1$ in $\rho_1$ is final, after the replacement, the state that occurs after $j-1$ letters are processed after position $s_0$ in $\rho$ is final as well.
However the $n^\text{th}$ letter from the end of the word processed by this accepting run of $\aut$ is a $0$, contradicting that $\aut$ recognises $L_n$.
Thus we have that $|Q| \cdot |\Gamma|$ is at least equal to the number of rotationally equivalent classes, that is, $|Q| \cdot |\Gamma| \geqslant \frac{2^n}{n}$.
Thus the size of $\aut$ is at least $(\frac{2^n}{n})^{1/2}$.
\end{proof}

\subsubsection{Proof of Theorem~\ref{theorem:succinct_VPA}}

Recall that we need to prove that \HD-VPA can be exponentially more succinct than DVPA and that VPA can be exponentially more succinct than \HD-VPA.
We split the proof into two parts.

\begin{lemma}
\HD-VPA can be exponentially more succinct than DVPA.
\end{lemma}
\begin{proof}
We construct a family~$(C_n')_{n \in \nats}$ of languages
such that there is an \HD-VPA
of size~$O(n)$ recognising $C_n'$,
yet every DVPA recognising $C_n'$ has at least exponential size in $n$.
This family is obtained by adapting
the family $(C_n)_{n \in\nats}$ that we used to prove
the succinctness of \HD-PDA in Section \ref{section_succinctness}:
Once again, we consider
the word $c_n\in (\$\{0,1\}^n)^*$ describing
an $n$-bit binary counter counting from $0$ to $2^{n}-1$.
We consider the languages~$C_n' \subseteq \{0,1,\$,\#\}^*$ of bad counters, where $0$, $1$ and $\$$ are call symbols and
$\#$ is a return symbol:
\[
C_n'= \big\{w \in \{0,1,\$,\#\}^*| w \neq c_n\#^{2^n(n+1)}\big\}
\]
The only difference with $C_n$
is that the forbidden word is $c_n\#^{2^n(n+1)}$
instead of $c_n\#$.
An \HD-VPA of size $O(n)$ recognising $C_n'$
is obtained by a small modification of the construction
presented in the proof of 
Lemma \ref{lemma:succinct_GFGPDA1}.
We adapt the construction of the automaton~$\aut$
recognising $C_n$ as follows:
\begin{itemize}
    \item 
    The push phase is identical;
    \item 
    The check phase is performed
    by consuming the $\#$ symbols
    instead of having $\epsilon$-transitions.
    While the stack is not empty,
    $\aut$ accepts even if it has not
    found evidence of bad counting yet.
    Moreover, $\aut$ transitions towards a final sink state
    if a non-$\#$ symbol is read.
    Once the stack is empty, it transitions towards
    the final phase;
    \item 
    In the final phase,
    since the prefix processed up to this point
    ends with an empty stack,
    if the suffix left to read is non-empty
    then the input is not equal to $c_n\#^{2^n(n+1)}$,
    and can be accepted.
\end{itemize}

Finally, we can prove 
that every DPDA (and in particular every DVPA)
recognising $C_n'$
has at least exponential size in $n$
in the exact same way as we proved
Lemma~\ref{lemma:succinct_GFGPDA2}:
The proof only uses the fact that $c_n$
is an infix of the single word rejected by $C_n$, 
% and ignores the $\#$ symbols,
thus $C_n'$ can be treated identically.
Note that this lower bound is independent
of the partition of the letters
into calls, returns, and internals.
\end{proof}


\begin{lemma}
\label{lemma_vpavsgfgvpa}
VPA can be exponentially more succinct than \HD-VPA.
\end{lemma}

We show that there exists a family~$(L'_n)_{n \in \nats}$ of languages such that there exists a VPA of size~$O(n)$  recognising $L_n'$ while every \HD-VPA recognising the same language has size at least $2^{n/6}$.

Towards this we consider a language $L'_n$ of words in $ (01+10)^* \cdot (\epsilon+0+1)$ with the $n^\text{th}$ last letter being $1$.
We first note that $L'_n$ can be recognised by a  VPA with $O(n)$ states, which checks that the input is in $(01+10)^* \cdot (\epsilon+0+1)$ and nondeterministically guesses the $n^{\text{th}}$ last letter and verifies that it is a $1$.


First, we claim that every DFA recognising $L'_n$ has exponential size.

\begin{remark} \label{rem:GFG_Ln_DFA}
Every DFA recognising $L'_n$ has at least $2^{\lceil n /2 \rceil}$ states.
\end{remark}


Using this, we obtain an exponential lower bound on the size of \HD-VPA recognising $L_n'$, thereby completing the proof of Lemma~\ref{lemma_vpavsgfgvpa}.

\begin{lemma}
Every \HD-VPA recognising $L'_n$ has at least size~$2^{\lceil n/6 \rceil}$.
\end{lemma}

\begin{proof}
The proof is based on the fact that \HD-NFA can be determinised by pruning~\cite{BKS17}, that is, they always contain an equivalent DFA, i.e. the lower bound of Remark~\ref{rem:GFG_Ln_DFA} is applicable to \HD-NFA as well.

Let $\aut$ be an \HD-VPA recognising $L_n'$.
We consider the following cases:
\begin{enumerate}
    \item \emph{Both $0$ and $1$ are either a return symbol or an internal symbol}: The \HD-VPA $\aut$ in this case can essentially be seen as an \HD-NFA with the same set of states, since the stack is not used (it is always equal to $\bot$).
    Given that \HD-NFA are determinisable by pruning, by Remark~\ref{rem:GFG_Ln_DFA} such an \HD-NFA has at least $2^{\lceil n/2 \rceil}$ states.
    \item \emph{At least one of $0$ and $1$ is a call symbol while the other one is a call or an internal symbol}: Let $Q$ be the set of states and $\Gamma$ be the stack alphabet of $\aut$.
    Since the height of the stack is nondecreasing, $\aut$ has only access to the top stack symbol.
    We can thus construct an equivalent \HD-NFA over finite words with states in $Q \times \Gamma$.
    Since \HD-NFA are determinizable by pruning, and using Remark \ref{rem:GFG_Ln_DFA} again, we have that $|Q| \cdot |\Gamma| \geqslant 2^{\lceil n/2 \rceil}$.
    Thus either $|Q| \geqslant 2^{n/4}$ or $|\Gamma| \geqslant 2^{n/4}$.
    Hence for this case, we have that the size of the \HD-VPA is at least $2^{n/4}$.
    \item \emph{One of $0$ and $1$ is a call symbol while the other one is a return symbol}: Note that since a word in $L_n'$ is composed of sequences of $10$ and $01$, the stack height can always be restricted to $2$.
    Thus the configuration space of $\aut$, restricted to configurations on accepting runs, is finite, and there is an equivalent \HD-NFA of size at most $|Q| \cdot |\Gamma|^2$.
    Thus $|Q| \cdot |\Gamma|^2 \geqslant 2^{\lceil n/2 \rceil}$ giving either $|Q| \geqslant 2^{\lceil n/6 \rceil}$ or $|\Gamma| \geqslant 2^{\lceil n/6 \rceil}$.
    Again by the determinizability by pruning argument, we have that the size of the \HD-VPA $\aut$ is at least $2^{\lceil n/6 \rceil}$.
\qedhere
\end{enumerate}
\end{proof}



==> content/vpa_resolver.tex <==

Finally, for \HD-VPA, the situation is again  much better. The classical game-based characterisation of \HDness of $\omega$-regular automata by Henzinger and Piterman~\cite{HP06} can be lifted to VPA and is, crucially, decidable.

\begin{theorem}
\label{theorem_visiblyresolver}
Every \HD-VPA has a (visibly) pushdown resolver.
\end{theorem}


